LogicBench: Towards Systematic Evaluation of Logical Reasoning Ability of Large Language Models

Recently developed large language models (LLMs) have been shown to perform remarkably well on a wide range of language understanding tasks. But, can they really "reason" over the natural language? This question has been receiving significant research attention and many reasoning skills such as commonsense, numerical, and qualitative have been studied. However, the crucial skill pertaining to 'logical reasoning' has remained underexplored. Existing work investigating this reasoning ability of LLMs has focused only on a couple of inference rules (such as modus ponens and modus tollens) of propositional and first-order logic. Addressing the above limitation, we comprehensively evaluate the logical reasoning ability of LLMs on 25 different reasoning patterns spanning over propositional, first-order, and non-monotonic logics. To enable systematic evaluation, we introduce LogicBench, a natural language question-answering dataset focusing on the use of a single inference rule. We conduct detailed analysis with a range of LLMs such as GPT-4, ChatGPT, Gemini, Llama-2, and Mistral using chain-of-thought prompting. Experimental results show that existing LLMs do not fare well on LogicBench; especially, they struggle with instances involving complex reasoning and negations. Furthermore, they sometimes overlook contextual information necessary for reasoning to arrive at the correct conclusion. We believe that our work and findings facilitate future research for evaluating and enhancing the logical reasoning ability of LLMs. Data and code are available at https://github.com/Mihir3009/LogicBench.

==> tables/CoT_table.tex <==
\begin{table}[!htp]\centering
\centering
\small
\resizebox{0.85\linewidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c}\toprule
& &\multicolumn{3}{c}{GPT-3} &\multicolumn{3}{|c}{ChatGPT} \\ \midrule
Type & Axiom & $A(No)$ & $A(Yes)$ & $Acc$ & $A(No)$ & $A(Yes)$ & $Acc$ \\ \midrule 
\multirow{8}{*}{PL} & DD  &80.4 &37.5 &67.5 &89.3 &58.3 &80 \\ 
& HS &100 &43.5 &67.5 &100 &66.7 &87.5 \\
& MT &90.2 &41 &66.2 &86.4 &78.6 &85 \\
& BD &86.5 &46.4 &72.5 &85.5 &61.1 &80 \\
& MI &100 &26.7 &31.2 &69.5 &9.5 &53.8 \\
& DS &75.4 &27.3 &68.8 &74.7 &0 &73.8 \\
& CD &94.4 &40.9 &65 &91.7 &75 &87.5 \\
& CT &97.8 &55.9 &80 &100 &55.6 &80 \\ \midrule
\textbf{Avg} &\textbf{} &\textbf{90.6} &\textbf{39.9} &\textbf{64.8} &\textbf{87.1} &\textbf{50.6} &\textbf{78.4} \\ \midrule \midrule
\multirow{9}{*}{FOL} & DD &73.8 &20 &63.7 &80.4 &34.5 &63.7 \\ 
& MP &93.3 &58 &71.2 &81.5 &80.8 &81.2 \\
& HS &100 &52.6 &77.5 &87.9 &59.1 &80 \\
& MT &82.6 &35.3 &62.5 &83.1 &88.9 &83.8 \\
& BD &79.7 &43.8 &72.5 &87.5 &75 &85 \\
& UI &100 &80 &87.5 &83.3 &100 &90 \\
& EI &86.4 &94.4 &90 &62.5 &100 &70 \\
& DS &80.8 &85.7 &81.2 &75 &0 &75 \\
& CD &95.7 &51.6 &75 &90.5 &82.4 &88.8 \\ \midrule
\textbf{Avg} &\textbf{} &\textbf{88} &\textbf{57.9} &\textbf{75.7} &\textbf{81.3} &\textbf{69} &\textbf{79.7} \\ \midrule \midrule
\multirow{8}{*}{NM} & RAP &68.9 &74.3 &71.2 &50 &0 &50 \\
& RE3 &51.9 &53.8 &52.5 &50 &50 &50 \\
& RE2 &48.7 &0 &47.5 &55.6 &100 &60 \\
& DRS &66.1 &4.2 &47.5 &68.8 &0 &55 \\
& DRI &59.1 &61.1 &60 &44.4 &0 &40 \\
& RE1 &72.3 &13.3 &61.3 &73.3 &0 &68.8 \\
& DRO &63.2 &61.9 &62.5 &50 &0 &50 \\
& DRD &87.5 &59.4 &65 &51.3 &100 &52.5 \\ \midrule
\textbf{Avg} &\textbf{} &\textbf{64.7} &\textbf{41} &\textbf{58.4} &\textbf{55.4} &\textbf{31.2} &\textbf{53.3} \\ 
\bottomrule
\end{tabular}
}
\vspace{0.2cm}
\caption{Performance of GPT-3 and ChatGPT in Chain-of-Thought (CoT) setting in terms of label-wise accuracy on LogicBench(Eval), where A(Yes) and A(No) denote the accuracy for the Yes and No labels, respectively. $Acc$ denotes combined accuracy.}
\label{tab:cot_results}
\end{table}

==> tables/acc_sd.tex <==
% Table generated by Excel2LaTeX from sheet 'FLAN-T5'
\begin{table}
  \centering
    \resizebox{0.9\linewidth}{!}{
    
    \begin{tabular}{c|c|c|c|c|c|c} \toprule
      Type    &    Axiom  & FLAN-T5 & Tk-instruct & UnifiedQA & GPT-3 & ChatGPT \\ 
      \midrule
      
    \multirow{8}[0]{*}{PL} 
          & HS & $73.3_{0.0072}$ & $81.2_{0.0375}$ & $82.1_{0.0505}$ & $91.7_{0.0361}$ & $81.2_{0.0125}$ \\
          & DS & $34.6_{0.1449}$ & $47.9_{0.0753}$ & $54.6_{0.0191}$ & $75.4_{0.01909}$ & $69.6_{0.01909}$ \\
          
          & CD & $31.7_{0.0629}$ & $40.8_{0.1264}$ & $35.8_{0.0887}$ & $90_{0.0433}$ & $93.8_{0.0216}$  \\
          
          & DD & $62.5_{0.0433}$ & $67.5_{0.0866}$ & $6.7_{0.0288}$ & $73.3_{0.0072}$ & $49.2_{0.0688}$ \\
          
          & BD & $28.3_{0.0144}$ & $50.4_{0.1120}$ & $12.9_{0.0144}$ & $81.2_{0.0433}$ & $81.2_{0.0216}$ \\
          & MT & $70_{0.0125}$ & $56.2_{0.025}$ & $58.3_{0.0144}$ & $56.7_{0.0361}$ & $70.8_{0.0191}$\\
          
          & MI & $28.7_{0.0125}$ & $45_{0.0433}$ & $26.2_{0}$ & $60.4_{0.0361}$ & $66.7_{0.0473}$ \\
          & CT & $41.7_{0.2886}$ & $47.1_{0.2093}$ & $12.1_{0.0505}$ & $95.8_{0.0191}$ & $77.1_{0.0315}$ \\ \midrule
          & \textbf{Avg} &$\textbf{46.4}_\textbf{0.0733}$ & $\textbf{54.5}_\textbf{0.0894}$ & $\textbf{36.1}_\textbf{0.0333}$ & $\textbf{73.5}_\textbf{0.0283}$ & $\textbf{73.7}_\textbf{0.0302}$ \\  \midrule\midrule

    \multirow{9}[0]{*}{FOL} 
          & EI & $100_{0}$ & $95_{0.0433}$ & $99.2_{0.0144}$ & $93.3_{0.0577}$ & $94.2_{0.0288}$ \\
          & UI & $91.7_{0.0288}$ & $86.7_{0.0144}$ & $79.2_{0.0288}$ & $92.5_{0.025}$ & $89.2_{0.0144}$ \\
          & MP & $89.6_{0.0072}$ & $86.2_{0.0216}$ & $73.3_{0.0144}$ & $81.7_{0.0144}$ & $85_{0.0216}$ \\
          & HS & $74.2_{0.0072}$ & $76.7_{0.0072}$ & $84.2_{0.0382}$ & $90.4_{0.0260}$ & $77.5_{0.0216}$ \\
          & DS & $51.7_{0.1993}$ & $61.3_{0.0331}$ & $76.7_{0.0144}$ & $82.9_{0.0382}$ & $89.6_{0.0072}$ \\
          & CD & $33.3_{0.0382}$ & $73.8_{0.3473}$ & $15.8_{0.0402}$ & $83.8_{0.0451}$ & $92.1_{0.0191}$ \\ 
          & DD& $55_{0.05}$ & $40.4_{0.0260}$ & $4.2_{0.0260}$ &$75_{0.0125}$ & $54.2_{0.0591}$  \\
          & BD & $25.8_{0.0144}$ & $64.2_{0.3068}$ & $5.8_{0.0260}$ & $77.9_{0.0191}$ & $87.1_{0.0439}$  \\
          & MT & $73.3_{0.0144}$ & $62.5_{0.0451}$ & $54.2_{0.0072}$ & $67.9_{0.0402}$ & $70_{0.0866}$ \\ \midrule
          & \textbf{Avg} & $\textbf{66.1}_\textbf{0.0399}$ & $\textbf{71.9}_\textbf{0.0939}$ & $\textbf{54.7}_\textbf{0.0233}$ & $\textbf{82.8}_\textbf{0.0309}$ & $\textbf{82.1}_\textbf{0.0336}$  \\  \midrule\midrule
    
    \multirow{8}[0]{*}{NM} 
          & DRI & $60_{0.025}$ & $53.3_{0.0803}$ & $56.7_{0.0382}$ & $83.3_{0.0144}$ & $80.8_{0.0288}$ \\ 
          & DRS & $48.3_{0.0072}$ & $37.1_{0.0520}$ & $50_{0.0451}$ & $64.2_{0.0402}$ & $66.7_{0.0144}$  \\
          & DRD & $95_{0}$ & $79.2_{0.0946}$ & $71.7_{0.0722}$ & $90.8_{0.0382}$ & $89.2_{0.0144}$ \\
          & DRO & $41.7_{0.0382}$ & $44.2_{0.0764}$ & $54.2_{0.0144}$ & $73.3_{0.0382}$ & $76.7_{0.1665}$ \\
          & RE1 & $55.8_{0.0617}$ & $41.7_{0.0260}$ & $75_{0.0125}$ & $72.5_{0.025}$ & $60.4_{0.0732}$  \\
          & RE2 &$100_{0}$ & $95.8_{0.0382}$ & $54.2_{0.1377}$ & $50_{0}$ & $63.3_{0.1010}$ \\
          & RE3 & $64.2_{0.0289}$ & $61.7_{0.0722}$ & $79.2_{0.0144}$ & $71.7_{0.0144}$ & $72.5_{0.05}$  \\
          & RAP & $65.4_{0.0473}$ & $82.9_{0.0144}$ & $67.5_{0.0545}$ & $61.7_{0.0072}$ & $64.2_{0.0260}$ \\ \midrule
          & \textbf{Avg} & $\textbf{66.3}_\textbf{0.0260}$ & $\textbf{62}_\textbf{0.0568}$ & $\textbf{63.5}_\textbf{0.0486}$ & $\textbf{70.9}_\textbf{0.0222}$ & $\textbf{71.7}_\textbf{0.0593}$ \\  \bottomrule
    \end{tabular}%
    }
    \vspace{0.2cm}
    \caption{Average and standard deviation across three different prompts corresponding to each inference rule for Table 5 (main paper).}
    \label{tab:acc_sd}%
\end{table}%



% \begin{table}[!htp]\centering
% \caption{Generated by Spread-LaTeX}\label{tab: }
% \scriptsize
% \begin{tabular}{lrrrrrrrrrrrr}\toprule
% & &\multicolumn{2}{c}{FLAN-T5} &\multicolumn{2}{c}{Tk-instruct} &\multicolumn{2}{c}{UnifiedQA} &\multicolumn{2}{c}{GPT-3} &\multicolumn{2}{c}{ChatGPT} \\
% type &axiom &mean\_acc &std\_acc &mean\_acc &std\_acc &mean\_acc &std\_acc &mean\_acc &std\_acc &mean\_acc &std\_acc \\
% \multirow{8}{*}{PL} &hypothetical\_syllogism 

% &disjunctive\_syllogism 

% &constructive\_dillema 

% &destructive\_dillema 

% &bidirectional\_dilemma 

% &modus\_tollens 

% &material\_implication 

% &commutation 

% \textbf{Avg} &\textbf{} &\textbf{46.4} &\textbf{0.0733025186160643} &\textbf{54.5} &\textbf{0.089440713755} &\textbf{36.1} &\textbf{0.033318484435000004} &\textbf{73.5} &\textbf{0.028356199518999998} &\textbf{73.7} &\textbf{0.030201989065} \\

% & & & & & & & & & & & \\
% \multirow{9}{*}{FOL} &existential\_instantiation \\

% &universal\_instantiation \\

% &modus\_ponens &\\ 

% &hypothetical\_syllogism \\ 

% &disjunctive\_syllogism \\

% &constructive\_dillema \\

% &destructive\_dillema \\

% &bidirectional\_dilemma \\

% &modus\_tollens \\

% \textbf{Avg} &\textbf{} &\textbf{66.1} &\textbf{0.03996720107111111} &\textbf{71.9} &\textbf{0.09387297217722221} &\textbf{54.7} &\textbf{0.023310813439444446} &\textbf{82.8} &\textbf{0.030913674882222224} &\textbf{82.1} &\textbf{0.03360969746055556} \\
% & & & & & & & & & & & \\


% \multirow{8}{*}{NM} &default\_reasoning\_irr &\\

% &default\_reasoning\_several \\

% &default\_reasoning\_default &\\

% &default\_reasoning\_open \\

% &reasoning\_about\_exceptions\_1 \\

% &reasoning\_about\_exceptions\_2 \\

% &reasoning\_about\_exceptions\_3 \\

% &reasoning\_about\_priority  \\

% \textbf{Avg} &\textbf{} \\
% \bottomrule
% \end{tabular}
% \end{table}

==> tables/axiom_examples.tex <==
% % Table generated by Excel2LaTeX from sheet 'Examples'
% \begin{table}[htbp]
%   \centering
%   \caption{Add caption}
%   % \resizebox{\linewidth}{!}{
%     \begin{tabular}{c|c|c} \toprule
%     type  & axiom & \multicolumn{1}{l}{Examples} \\ \midrule
%     \multirow{16}[0]{*}{PL} & \multirow{2}[0]{*}{hypothetical\_syllogism} & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ 
%           &       & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ 
%           & \multirow{2}[0]{*}{disjunctive\_syllogism} & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ 
%           &       & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular} \\ 
%           & \multirow{2}[0]{*}{constructive\_dillema} & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ 
%           &       & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular} \\
%           & \multirow{2}[0]{*}{destructive\_dillema} & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ 
%           &       & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular} \\ 
%           & \multirow{2}[0]{*}{bidirectional\_dilemma} & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ 
%           &       & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular} \\
%           & \multirow{2}[0]{*}{modus\_tollens} &\begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ 
%           &       & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular} \\
%           & \multirow{2}[0]{*}{material\_implication} & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ 
%           &       & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular} \\
%           & \multirow{2}[0]{*}{commutation} & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ 
%           &       & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular} \\  \midrule \midrule
%     \multirow{18}[0]{*}{FOL} & \multirow{2}[0]{*}{existential\_instantiation} & Context: \newline{}Question:  \\
%           &       & Context: \newline{}Question:  \\
%           & \multirow{2}[0]{*}{universal\_instantiation} & Context: \newline{}Question:  \\
%           &       & Context: \newline{}Question:  \\
%           & \multirow{2}[0]{*}{modus\_ponens} & Context: \newline{}Question:  \\
%           &       & Context: \newline{}Question:  \\
%           & \multirow{2}[0]{*}{hypothetical\_syllogism} & Context: \newline{}Question:  \\
%           &       & Context: \newline{}Question:  \\
%           & \multirow{2}[0]{*}{disjunctive\_syllogism} & Context: \newline{}Question:  \\
%           &       & Context: \newline{}Question:  \\
%           & \multirow{2}[0]{*}{constructive\_dillema} & Context: \newline{}Question:  \\
%           &       & Context: \newline{}Question:  \\
%           & \multirow{2}[0]{*}{destructive\_dillema} & Context: \newline{}Question:  \\
%           &       & Context: \newline{}Question:  \\
%           & \multirow{2}[0]{*}{bidirectional\_dilemma} & Context: \newline{}Question:  \\
%           &       & Context: \newline{}Question:  \\
%           & \multirow{2}[0]{*}{modus\_tollens} & Context: \newline{}Question:  \\
%           &       & Context: \newline{}Question:  \\ \midrule \midrule
%     \multirow{16}[0]{*}{NM} & \multirow{2}[0]{*}{default\_reasoning\_irr} & Context: \newline{}Question:  \\
%           &       & Context: \newline{}Question:  \\
%           & \multirow{2}[0]{*}{default\_reasoning\_several} & Context: \newline{}Question:  \\
%           &       & Context: \newline{}Question:  \\
%           & \multirow{2}[0]{*}{default\_reasoning\_default} & Context: \newline{}Question:  \\
%           &       & Context: \newline{}Question:  \\
%           & \multirow{2}[0]{*}{default\_reasoning\_open} & Context: \newline{}Question:  \\
%           &       & Context: \newline{}Question:  \\
%           & \multirow{2}[0]{*}{reasoning\_about\_exceptions\_1} & Context: \newline{}Question:  \\
%           &       & Context: \newline{}Question:  \\
%           & \multirow{2}[0]{*}{reasoning\_about\_exceptions\_2} & Context: \newline{}Question:  \\
%           &       & Context: \newline{}Question:  \\
%           & \multirow{2}[0]{*}{reasoning\_about\_exceptions\_3} & Context: \newline{}Question:  \\
%           &       & Context: \newline{}Question:  \\
%           & \multirow{2}[0]{*}{reasoning\_about\_priority} & Context: \newline{}Question:  \\
%           &       & Context: \newline{}Question:  \\ \bottomrule
%     \end{tabular}%
%     % }
%   \label{tab:addlabel}%
% \end{table}%


% Table generated by Excel2LaTeX from sheet 'Examples'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
  \resizebox{\linewidth}{!}{
  % \resizebox{0.7\textwidth}{!}{
    \begin{tabular}{c|c|c} \toprule \toprule
    type  & axiom & example \\ \midrule
    \multirow{8}[0]{*}{PL} & hypothetical\_syllogism &  \begin{tabular}[c]{@{}l@{}}Context: If Katie finishes all her homework, then she can go to the party. \\ If she is at the party, then she will be drunk.\\ Question: If Katie finishes her homework, does that imply she is drunk? \end{tabular}  \\ \cmidrule{2-3}
          & disjunctive\_syllogism &  \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}\\ \cmidrule{2-3}
          & constructive\_dillema & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ \cmidrule{2-3}
          & destructive\_dillema & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ \cmidrule{2-3}
          & bidirectional\_dilemma & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ \cmidrule{2-3}
          & modus\_tollens &  \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ \cmidrule{2-3}
          & material\_implication & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ \cmidrule{2-3}
          & commutation & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ \midrule\midrule
    \multirow{9}[0]{*}{FOL} & existential\_instantiation & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ \cmidrule{2-3}
          & universal\_instantiation & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ \cmidrule{2-3}
          & modus\_ponens & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ \cmidrule{2-3}
          & hypothetical\_syllogism & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ \cmidrule{2-3}
          & disjunctive\_syllogism & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ \cmidrule{2-3}
          & constructive\_dillema & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ \cmidrule{2-3}
          & destructive\_dillema & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ \cmidrule{2-3}
          & bidirectional\_dilemma & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ \cmidrule{2-3}
          & modus\_tollens & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ \midrule\midrule
    \multirow{8}[0]{*}{NM} & default\_reasoning\_irr & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ \cmidrule{2-3}
          & default\_reasoning\_several & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ \cmidrule{2-3}
          & default\_reasoning\_default & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ \cmidrule{2-3}
          & default\_reasoning\_open & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ \cmidrule{2-3}
          & reasoning\_about\_exceptions\_1 & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ \cmidrule{2-3}
          & reasoning\_about\_exceptions\_2 & \begin{tabular}[c]{@{}l@{}}Context: \\ Question:\end{tabular}  \\ \cmidrule{2-3}
          & reasoning\_about\_exceptions\_3 & \begin{tabular}[c] {@{}l@{}}Context: \\ Question:\end{tabular}  \\ \cmidrule{2-3}
          & reasoning\_about\_priority & \begin{tabular}[c] {@{}l@{}}Context: \\ Question:\end{tabular}  \\ \bottomrule \bottomrule
    \end{tabular}%
    }
  \label{tab:addlabel}%
\end{table}%


==> tables/bard_gpt4.tex <==
\begin{table}
\centering
\footnotesize
\resizebox{0.5\linewidth}{!}{
    \begin{tabular}{c|c} \toprule
        \textbf{Logic}   & \textbf{Bard}  \\ \midrule
        PL      & 65.0\% \\
        FOL     & 71.1\% \\
        NM      & 15.0\% \\ \midrule
        Average & 51.2\% \\ \bottomrule
    \end{tabular}
}
\caption{Case study of performance of BARD on a subset of \textit{LogicBench}}
\label{tab:bard_gpt4}
\end{table}

==> tables/cross_task_analysis.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}
\centering
\footnotesize
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{c|ccc}
\toprule
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Model \\ Training\end{tabular}}} & \multicolumn{3}{c}{\textbf{Model Evaulation}}                                     \\ \cmidrule{2-4} 
                                                                                    & \multicolumn{1}{c|}{\textbf{PL}} & \multicolumn{1}{c|}{\textbf{FOL}} & \textbf{NM} \\ \midrule
PL                                                                                  & \multicolumn{1}{c|}{93.13}       & \multicolumn{1}{c|}{86.25}        & 49.09       \\ 
FOL                                                                                 & \multicolumn{1}{c|}{86.72}       & \multicolumn{1}{c|}{97.34}        & 54.73       \\ 
NM                                                                                  & \multicolumn{1}{c|}{43.28}       & \multicolumn{1}{c|}{57.66}        & 92.73       \\ \bottomrule
\end{tabular}
}
\caption{Results on cross-type logic using T5-Large.}
\label{tab:cross_type_logic}
\end{table}

==> tables/explanation_example_1.tex <==
\begin{table}[]
  \centering
  \resizebox{\linewidth}{!}{
  \fontsize{13pt}{13pt}\selectfont
  % \resizebox{\textwidth}{!}{
    \begin{tabular}{m{1.1cm}|m{5cm}|m{4cm}|c|m{12cm}} \toprule
    
	Type & Context & Question & Answer & Logical Steps \\ \midrule
	PL (DS) & We know that at  least one of the following is true (1) she is not making a cake for the party and (2) he is writing a report for his boss. Note that we do not know which ones of (1) and (2) are true. It might be the case that only (1) is true, or only (2) is true or both are true. & If she is making a cake for the party, does this mean that he is writing a report for his boss? & Yes   & \textbf{Prediction:} No. \newline \newline Logical reasoning steps: 
    \begin{enumerate}
        \item We are given two possibilities: either she is not making a cake for the party (denoted as statement 1) or he is writing a report for his boss (denoted as statement 2).
        \item We are not given any information that directly connects the two statements or suggests that they are dependent on each other.
        \item Therefore, the presence or absence of her making a cake does not provide any conclusive information about whether he is writing a report.
        \item Without further evidence or a clear relationship between the statements, we cannot infer that if she is making a cake, he must be writing a report.
        \item Hence, the answer to the question "If she is making a cake for the party, does this mean that he is writing a report for his boss?" is "No."
    \end{enumerate}
     \\ \midrule 
     
	FOL (DD) & If someone takes care of her health, then they will be fit and healthy. If they indulge in unhealthy habits, then they will be prone to diseases. We know that atleast one of the following is true (1) Jenny won't be fit and healthy and (2) she won't be prone to diseases. Note that we do not know which ones of (1) and (2) are true. It might be the case that only (1) is true, or only (2) is true or both are true. & If at least one of (1) and (2) is true, can we say, at least one of the following must always be true? (a) jenny doesn't take care of her health and (b) she doesn't indulge in unhealthy habits & Yes   & \textbf{Prediction:} No, we cannot say that at least one of the following must always be true: (a) Jenny doesn't take care of her health, and (b) she doesn't indulge in unhealthy habits.\newline \newline Logical Reasoning Steps: 
    \begin{enumerate}
        \item If someone takes care of their health, they will be fit and healthy. This implies that if Jenny takes care of her health, she will be fit and healthy.
        \item If someone indulges in unhealthy habits, they will be prone to diseases. This implies that if Jenny indulges in unhealthy habits, she will be prone to diseases.
        \item We are given that at least one of the following is true: (1) Jenny won't be fit and healthy, or (2) she won't be prone to diseases. This means that it could be the case that only (1) is true, only (2) is true, or both are true.
        \item If only (1) is true, it means Jenny won't be fit and healthy, but we don't know if she takes care of her health or indulges in unhealthy habits.
        \item If only (2) is true, it means Jenny won't be prone to diseases, but we don't know if she takes care of her health or indulges in unhealthy habits.
        \item If both (1) and (2) are true, it means Jenny won't be fit and healthy and won't be prone to diseases, but we still don't know if she takes care of her health or indulges in unhealthy habits.
        \item Therefore, we cannot conclude that at least one of the following must always be true: (a) Jenny doesn't take care of her health, and (b) she doesn't indulge in unhealthy habits.
    \end{enumerate} \\  \midrule
    
    NM (DRS) & John and Mary are parents. parents are usually loving and supportive. parents are normally responsible. Mary isn't loving and supportive. John is not responsible. & Does this imply that Mary is responsible and John is loving and supportive? & Yes  & \textbf{Prediction:} No, this context does not imply that Mary is responsible and John is loving and supportive.\newline{}\newline{} Logical Reasoning Steps:
    \begin{enumerate}
        \item The context states that parents are usually loving and supportive, and parents are normally responsible.
        \item However, it also mentions that Mary isn't loving and supportive and John is not responsible.
        \item Since the context specifies that Mary isn't loving and supportive, it contradicts the assumption that Mary is responsible.
        \item Similarly, the context specifies that John is not responsible, which contradicts the assumption that John is loving and supportive.
        \item Therefore, based on the given context, we cannot conclude that Mary is responsible or that John is loving and supportive. 
    \end{enumerate} 
    \\ \bottomrule
	\end{tabular}%
    }
    \vspace{0.2cm}
  \caption{Step-by-step reasoning for selected axioms from all three logic types.}
  \label{tab:reasoning_steps}%
\end{table}%


==> tables/first_order_results.tex <==
\begin{table*}[]
\centering
\begin{tabular}{|c|cc|cc|cc|cc|}
\hline
\multirow{2}{*}{Logic Axiom}                                        & \multicolumn{2}{c|}{GPT-3}              & \multicolumn{2}{c|}{LAMA}               & \multicolumn{2}{c|}{tk-instruct}        & \multicolumn{2}{c|}{FLAN-T5}            \\ \cline{2-9} 
                                                                    & \multicolumn{1}{c|}{Accuracy} & F-socre & \multicolumn{1}{c|}{Accuracy} & F-socre & \multicolumn{1}{c|}{Accuracy} & F-socre & \multicolumn{1}{c|}{Accuracy} & F-socre \\ \hline
\begin{tabular}[c]{@{}c@{}}Existential\\ Instantiation\end{tabular} & \multicolumn{1}{c|}{87.66\%}  & 87.59\% & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       \\ \hline
\begin{tabular}[c]{@{}c@{}}Universial\\ Instantiation\end{tabular}  & \multicolumn{1}{c|}{99.33\%}  & 99.33\% & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       \\ \hline
\begin{tabular}[c]{@{}c@{}}Modus\\ Ponens\end{tabular}              & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       \\ \hline
\begin{tabular}[c]{@{}c@{}}Modus\\ Tollens\end{tabular}             & \multicolumn{1}{c|}{69.67\%}  & 69.65\% & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       \\ \hline
\begin{tabular}[c]{@{}c@{}}Hypothetical\\ Syllogism\end{tabular}    & \multicolumn{1}{c|}{88.67\%}  & 88.66\% & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       \\ \hline
\begin{tabular}[c]{@{}c@{}}Disjunctive\\ Syllogism\end{tabular}     & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       \\ \hline
\begin{tabular}[c]{@{}c@{}}Destructive\\ Dillema\end{tabular}       & \multicolumn{1}{c|}{56\%}     & 55.95\% & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       \\ \hline
\begin{tabular}[c]{@{}c@{}}Constructive\\ Dillema\end{tabular}      & \multicolumn{1}{c|}{93.33\%}  & 93.30\% & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       \\ \hline
\begin{tabular}[c]{@{}c@{}}Bidirectional\\ Dillema\end{tabular}     & \multicolumn{1}{c|}{67.67\%}  & 65.86\% & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       \\ \hline
\end{tabular}
\caption{Evaluating LLMs on First-order Logic.}
\end{table*}

==> tables/llama_result.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{c|cc||c|cc||c|cc}
    \toprule
    \multicolumn{3}{c||}{\textbf{PL}} & \multicolumn{3}{c||}{\textbf{FOL}} & \multicolumn{3}{c}{\textbf{NM}} \\ \midrule
    \textbf{Rule} & \textbf{A(No)} & \textbf{A(Yes)} & \textbf{Rule} & \textbf{A(No)} & \textbf{A(Yes)} & \textbf{Rule} & \textbf{A(No)} & \textbf{A(Yes)} \\ \midrule
    
     HS & $88_{0.03}$  & $45_{0.35}$  & EG & $84_{0.06}$  & $79_{0.16}$  & DRI   & $49_{ 0.03}$  & $47_{0.11}$  \\
    
    DS & $73_{0.03}$  & $4_{0.06}$  & UI & $84_{0.1}$   & $63_{0.11}$  & DRS   & $73_{0.03}$  & $26_{0.22}$ \\
    
    CD & $80{0.07}$  & $29_{0.04}$  & MP & $82_{0.05}$  & $72_{0.33}$  & DRD   & $64_{0.02}$  & $57_{0.21}$ \\
    
    DD & $82_{0.05}$  & $3_{0.07}$   & HS & $83_{0.06}$  & $35_{0.02}$  & DRO   & $50_{ 0.05}$  & $49_{0.07}$  \\
    
    BD & $76_{0.02}$  & $27_{0.06}$ & DS & $83_{0.17}$  & $1_{0.03}$  & RE1   & $79_{0.05}$  & $30_{0.05}$  \\
    
    MT & $75_{0.02}$  & $25_{0.25}$  & CD & $72_{0.25}$  & $26_{0.02}$  & RE2   & $56_{0.18}$  & $58_{0.09}$\\
    
    MI & $75_{0}$     & $11_{0.19}$  & DD & $90_{0.09}$  & $25_{0.22}$   & RE3   & $50_{0.03}$  & $50_{0.04}$ \\
    
    CT &     $65_{0.07}$  & $9_{0.08}$  & BD & $86_{0.06}$  & $28_{0.03}$  & RAP   & $53_{0.04}$  & $60_{0.03}$ \\

    -     & - & - & MT & $78_{0.06}$  & $19_{0.01}$  & -     & - & - \\ \midrule
    
    \textbf{Avg} &    $\textbf{77}_{\textbf{0.04}}$ & $\textbf{22}_{\textbf{0.14}}$ & \textbf{Avg} & $\textbf{83}_{\textbf{0.1}}$ & $\textbf{39}_{\textbf{0.1}}$ & \textbf{Avg} & $\textbf{59}_{\textbf{0.05}}$ & $\textbf{47}_{\textbf{0.1}}$ \\ \bottomrule
    \end{tabular}%
    }
      \caption{Average and standard deviation across three different prompts corresponding to each inference rule for LLaMa-2-7B.}
  \label{tab:llama_2}%
\end{table}%


==> tables/logic_types.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{cccc}
\toprule
\multirow{2}{*}{\textbf{Axioms}}                                                   & \multicolumn{3}{c}{\textbf{Logic Type}}                                                                \\ \cmidrule{2-4} 
                                                                                        & \multicolumn{1}{c}{Propositional Logic} & \multicolumn{1}{c}{First-order Logic} & Non-monotonic Logic \\ \midrule
Modus Ponens                                                                            &X                 &\checkmark                &X                 \\ \midrule
\begin{tabular}[c]{@{}c@{}}Existential Instantiation\end{tabular}                     &X                 &\checkmark                &X                 \\ \midrule
\begin{tabular}[c]{@{}c@{}}Universal Instantiation\end{tabular}                       &X                 &\checkmark                &X                 \\ \midrule
Modus Tollens                                                                           &\checkmark                  &\checkmark                &X                 \\ \midrule
Hypothetical Syllogism                                                                  &\checkmark                  &\checkmark                &X                 \\ \midrule
Disjunctive Syllogism                                                                   &\checkmark                  &\checkmark                &X                 \\ \midrule
Constructive Dilemma                                                                    &\checkmark                  &\checkmark                &X                 \\ \midrule
Destructive Dilemma                                                                     &\checkmark                  &\checkmark                &X                 \\ \midrule
Bidirectional Dilemma                                                                   &\checkmark                  &\checkmark                &X                 \\ \midrule
Commutation                                                                             &\checkmark                  &X               &X                 \\ \midrule
Material Implication                                                                    &\checkmark                  &X              &X                 \\ \midrule
Default Reasoning                                                                       &X                 &X               &\checkmark                  \\ \midrule
\begin{tabular}[c]{@{}c@{}}Default Reasoning with\\ Irrelevant Information\end{tabular} &X                 &X               &\checkmark                  \\ \midrule
\begin{tabular}[c]{@{}c@{}}Default Reasoning with\\ Several Defaults\end{tabular}       &X                 &X               &\checkmark                  \\ \midrule
\begin{tabular}[c]{@{}c@{}}Default Reasoning with\\ Open Domain\end{tabular}            &X                 &X               &\checkmark                  \\ \midrule
\begin{tabular}[c]{@{}c@{}}Reasoning about Unknown\\ Exceptions 1\end{tabular}          &X                 &X               &\checkmark                  \\ \midrule
\begin{tabular}[c]{@{}c@{}}Reasoning about Unknown\\ Exceptions 2\end{tabular}          &X                 &X               &\checkmark                  \\ \midrule
\begin{tabular}[c]{@{}c@{}}Reasoning about Unknown\\ Exceptions 3\end{tabular}          &X                 &X               &\checkmark                  \\ \midrule
Reasoning about Priority                                                                &X                 &X               &\checkmark                  \\ 
\bottomrule
\end{tabular}
}
\vspace{0.2cm}
\caption{Comprehensive Representation of Logic Types in Covering Different Axioms, Showing the Number of Axioms Covered by Propositional Logic, First-Order Logic, and Non-Monotonic Logic, Respectively.}
\label{tab:logic_type}
\end{table}

==> tables/logical_FOL.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \resizebox{0.7\linewidth}{!}{
    \begin{tabular}{m{4.6cm}|m{3cm}|c|m{16cm}} \toprule
    % \begin{tabular}{m{4.5cm}|m{3cm}|c|m{15cm}} \toprule
    
    Context & Question & Answer & Logical Steps \\ \midrule
    
    % If someone takes care of her health, then they will be fit and healthy. If they indulge in unhealthy habits, then they will be prone to diseases. We know that atleast one of the following is true (1) Jenny won't be fit and healthy and (2) she won't be prone to diseases. Note that we do not know which ones of (1) and (2) are true. It might be the case that only (1) is true, or only (2) is true or both are true. & If at least one of (1) and (2) is true, can we say, at least one of the following must always be true? (a) Jenny doesn't take care of her health and (b) she doesn't indulge in unhealthy habits & Yes   & No, we cannot say that at least one of the following must always be true: (a) Jenny doesn't take care of her health, and (b) she doesn't indulge in unhealthy habits.\newline \newline Logical Reasoning Steps: 
    % \begin{enumerate}
    %     \item If someone takes care of their health, they will be fit and healthy. This implies that if Jenny takes care of her health, she will be fit and healthy.
    %     \item If someone indulges in unhealthy habits, they will be prone to diseases. This implies that if Jenny indulges in unhealthy habits, she will be prone to diseases.
    %     \item We are given that at least one of the following is true: (1) Jenny won't be fit and healthy, or (2) she won't be prone to diseases. This means that it could be the case that only (1) is true, only (2) is true, or both are true.
    %     \item If only (1) is true, it means Jenny won't be fit and healthy, but we don't know if she takes care of her health or indulges in unhealthy habits.
    %     \item If only (2) is true, it means Jenny won't be prone to diseases, but we don't know if she takes care of her health or indulges in unhealthy habits.
    %     \item If both (1) and (2) are true, it means Jenny won't be fit and healthy and won't be prone to diseases, but we still don't know if she takes care of her health or indulges in unhealthy habits.
    %     \item Therefore, we cannot conclude that at least one of the following must always be true: (a) Jenny doesn't take care of her health, and (b) she doesn't indulge in unhealthy habits.
    % \end{enumerate} \\ \midrule

    If someone buys a car , then they will save money on transportation . If they sell their car , then they will have more money to invest. We know that atleast one of the following is true (1) she won't save money on transportation and (2) she won't have more money to invest. Note that we do not know which ones of (1) and (2) are true. It might be the case that only (1) is true, or only (2) is true or both are true. & If at least one of (1) and (2) is true, can we say, at least one of the following must always be true? (a) sara didn't buy a car and (b) she didn't sell her car & Yes & No \newline Logical reasoning steps: \newline
    \begin{itemize}
        \item If someone buys a car, they will save money on transportation.
        \item If someone sells their car, they will have more money to invest.
        \item At least one of the following is true: (1) she won't save money on transportation and (2) she won't have more money to invest.
        \item We do not know which one of (1) and (2) is true, or if both are true.
        \item The question asks if at least one of (1) and (2) is true, can we say that at least one of the following must always be true: (a) Sara didn't buy a car and (b) she didn't sell her car.
        \item If (1) is true, it means Sara didn't save money on transportation. This does not necessarily mean she didn't buy a car or sell her car. Therefore, we cannot say that (a) must always be true.
        \item If (2) is true, it means Sara didn't have more money to invest. This does not necessarily mean she didn't buy a car or sell her car. Therefore, we cannot say that (b) must always be true.
        \item Based on the reasoning steps, the answer is No.
    \end{itemize} 
    \\ \midrule
    
    If someone takes a walk, then they will get fresh air. If they watch tv, then they will feel relaxed. We know that atleast one of the following is true (1) Jill won't get fresh air. and (2) she won't feel relaxed. Note that we do not know which ones of (1) and (2) are true. It might be the case that only (1) is true, or only (2) is true or both are true. & If at least one of (1) and (2) is true, can we say, at least one of the following must always be true? (a) Jill doesn't take a walk. and (b) she doesn't watch tv. & Yes   & No. Based on the given information, we cannot say that at least one of the following must always be true: (a) Jill doesn't take a walk, and (b) she doesn't watch TV.    \newline Logical Reasoning Steps:
    \begin{enumerate}
        \item If someone takes a walk, then they will get fresh air.
        \item If they watch TV, then they will feel relaxed.
        \item We know that at least one of the following is true: (1) Jill won't get fresh air, and (2) she won't feel relaxed.
        \item We do not know which one of (1) and (2) is true. It could be that only (1) is true, only (2) is true, or both are true.
        \item The question asks if at least one of (1) and (2) is true, can we say that at least one of the following must always be true: (a) Jill doesn't take a walk, and (b) she doesn't watch TV.
    \end{enumerate} \\ \midrule
    
    % If someone turns off the lights, then they will save electricity. If they use a generator, then they will pay a high electricity bill. We know that atleast one of the following is true (1) Linda won't save electricity and (2) she won't pay a high electricity bill. Note that we do not know which ones of (1) and (2) are true. It might be the case that only (1) is true, or only (2) is true or both are true. & If at least one of (1) and (2) is true, can we say, at least one of the following must always be true? (a) Linda doesn't turn off the lights and (b) she doesn't use a generator & Yes   & No, we cannot say that at least one of the following must always be true: (a) Linda doesn't turn off the lights and (b) she doesn't use a generator.\newline \newline Logical Reasoning Steps:
    % \begin{enumerate}
    %     \item From the given context, we have the following conditional statements:  If someone turns off the lights, then they will save electricity. If someone uses a generator, then they will pay a high electricity bill.
    %     \item We are also given that at least one of the following is true: (1) Linda won't save electricity. (2) Linda won't pay a high electricity bill.
    %     \item Let's consider the possibilities: If only (1) is true, it means Linda won't save electricity. This doesn't provide any information about whether Linda will turn off the lights or use a generator. If only (2) is true, it means Linda won't pay a high electricity bill. Again, this doesn't provide any information about whether Linda will turn off the lights or use a generator.
    %     \item If both (1) and (2) are true, it means Linda won't save electricity and won't pay a high electricity bill. This still doesn't provide any information about whether Linda will turn off the lights or use a generator.
    %     \item Since we don't have any specific information about whether Linda will turn off the lights or use a generator, we cannot conclude that at least one of the following must always be true: (a) Linda doesn't turn off the lights and (b) she doesn't use a generator. The given context doesn't establish a direct relationship between Linda's actions regarding turning off the lights or using a generator and statements (1) and (2). 
    % \end{enumerate} \\ \midrule

    If someone takes care of her health, then they will be fit and healthy. If they indulge in unhealthy habits, then they will be prone to diseases. We know that atleast one of the following is true (1) Jenny won't be fit and healthy and (2) she won't be prone to diseases. Note that we do not know which ones of (1) and (2) are true. It might be the case that only (1) is true, or only (2) is true or both are true. & If at least one of (1) and (2) is true, can we say, at least one of the following must always be true? (a) jenny doesn't take care of her health and (b) she doesn't indulge in unhealthy habits & Yes & No \newline Logical reasoning steps: \newline
    \begin{itemize}
        \item From the given context, we have two conditional statements:
        \begin{itemize}
            \item If someone takes care of her health, then they will be fit and healthy.
            \item If they indulge in unhealthy habits, then they will be prone to diseases.
        \end{itemize}
        \item We also know that at least one of the following is true:
        \begin{itemize}
            \item Jenny won't be fit and healthy.
            \item She won't be prone to diseases.
        \end{itemize}
        \item We are asked if we can conclude whether at least one of the following must always be true:
        \begin{itemize}
            \item Jenny doesn't take care of her health.
            \item She doesn't indulge in unhealthy habits.
        \end{itemize}
        \item Let's analyze the given options: \newline
        If Jenny is not fit and healthy [(1) is true], according to the first conditional statement, she might not be taking care of her health. So, (a) could be true. \newline
        If Jenny is not prone to diseases [(2) is true], according to the second conditional statement, she might not be indulging in unhealthy habits. So, (b) could be true.
        \item Based on the information provided in the context and the conditional statements, we cannot definitively conclude that at least one of the options (a) or (b) must always be true. It depends on the specific reasons for Jenny not being fit and healthy or not being prone to diseases.
    \end{itemize} 
    \\ \midrule
    
    If someone reads a lot, then they will get good grades. If they watch television, then they will have a sound sleep. We know that atleast one of the following is true (1) Jill won't get good grades and (2) she won't have a sound sleep. Note that we do not know which ones of (1) and (2) are true. It might be the case that only (1) is true, or only (2) is true or both are true. & If at least one of (1) and (2) is true, can we say, at least one of the following must always be true? (a) Jill doesn't read a lot and (b) she doesn't watch television & Yes   & No, we cannot say that at least one of the following must always be true: (a) Jill doesn't read a lot, and (b) she doesn't watch television.\newline \newline Logical Reasoning:
    \begin{enumerate}
       \item We know that if someone reads a lot, then they will get good grades.
    \item We also know that if someone watches television, then they will have a sound sleep.
    \item We are given that at least one of the following is true: (1) Jill won't get good grades and (2) she won't have a sound sleep.
    \item It is possible that only (1) is true, meaning Jill won't get good grades but she will have a sound sleep.
    \item It is also possible that only (2) is true, meaning Jill will get good grades but she won't have a sound sleep.
    \item It is also possible that both (1) and (2) are true, meaning Jill won't get good grades and she won't have a sound sleep.
    \item If only (1) is true, then it means Jill doesn't read a lot, but we don't know if she watches television or not.
    \item If only (2) is true, then it means Jill doesn't watch television, but we don't know if she reads a lot or not.
    \item If both (1) and (2) are true, then it means Jill doesn't read a lot and she doesn't watch television.
    \item Based on the given information, we cannot say for certain whether at least one of the following must always be true: (a) Jill doesn't read a lot and (b) she doesn't watch television.
    \end{enumerate}  \\ \midrule
    
     If someone takes a test, then they will get a good grade. If they do not revise enough, then they will not score well. We know that atleast one of the following is true (1) John won't get a good grade and (2) he will score well. Note that we do not know which ones of (1) and (2) are true. It might be the case that only (1) is true, or only (2) is true or both are true. & If at least one of (1) and (2) is true, can we say, at least one of the following must always be true? (a) john doesn't take a test and (b) he revises enough & Yes   & No \newline Logical reasoning steps: \newline
    \begin{enumerate}
        \item We know that if someone takes a test, they will get a good grade, which can be represented as: Test → Good Grade.
        \item We also know that if someone does not revise enough, they will not score well, which can be represented as: Not Enough Revision → Not Score Well.
        \item We are given that at least one of the following is true: (1) John won't get a good grade and (2) he will score well.
        \item This means that either Test → Good Grade is true (2 is true) or Not Enough Revision → Not Score Well is true (1 is true), or both are true.
        \item Now, let's analyze the implications of (a) and (b): \newline
        (a) John doesn't take a test: This statement is not directly provided in the context, so we cannot definitively say whether John takes the test or not based on the given information. \newline
        (b) He revises enough: This statement is also not directly provided in the context, so we cannot definitively say whether John revises enough based on the given information.
        \item In conclusion, based on the information provided in the context, we cannot determine whether (a) John doesn't take a test or (b) he revises enough. Therefore, we cannot say that at least one of these statements must always be true.
    \end{enumerate} 
    \\ \bottomrule
    \end{tabular}%
    }
    \vspace{0.2cm}
    \caption{Case study on generating a logical explanation for \textit{Destructive Dilemma} of \textit{first order logic} having the worst performance by \textit{ChatGPT} in this category}
  \label{tab:appendix_explain_FOL}%
\end{table*}%


==> tables/logical_NM.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \resizebox{1\linewidth}{!}{
    % \begin{tabular}{m{4.5cm}|m{3cm}|c|m{15.5cm}} \toprule
    \begin{tabular}{m{5cm}|m{4cm}|c|m{14.5cm}} \toprule
    Context & Question & Answer & Logical Steps \\ \midrule
    
    John and Mary are parents. parents are usually loving and supportive. parents are normally responsible. Mary isn't loving and supportive. John is not responsible. & Does this imply that Mary is responsible and John is loving and supportive? & Yes   & No \newline Logical Reasoning Steps:
    \begin{enumerate}
        \item The context states that parents are usually loving and supportive.
        \item The context also states that parents are normally responsible.
        \item The context further states that Mary isn't loving and supportive.
        \item The context states that John is not responsible.
        \item Based on the context, it can be inferred that Mary is not responsible because she is not loving and supportive.
        \item It can also be inferred that John is not loving and supportive because he is not responsible.
        \item Therefore, the context does not imply that Mary is responsible and John is loving and supportive.
    \end{enumerate} \\ \midrule
    
    apples and bananas are fruits. fruits are usually sweet. fruits are normally juicy. apples are not sweet. bananas are not juicy. & Does this mean that bananas are sweet and apples are juicy? & Yes   & No. \newline Logical Reasoning Steps:
    \begin{enumerate}
        \item According to the context, apples and bananas are fruits.
        \item The context also states that fruits are usually sweet and normally juicy.
        \item However, it is mentioned that apples are not sweet and bananas are not juicy.
        \item Therefore, based on the given information, we can conclude that bananas are not sweet and apples are not juicy.
        \item The question asks if bananas are sweet and apples are juicy.
        \item Based on the reasoning steps, the answer is No, bananas are not sweet and apples are not juicy.
    \end{enumerate} \\ \midrule
    
    cats and dogs are animals. animals have four legs. animals have fur. cats have no fur. dogs are not four-legged. & Does this mean that dogs have fur and cats have four legs? & Yes   & No. \newline Logical reasoning steps:
    \begin{enumerate}
        \item Cats and dogs are animals.
        \item Animals have four legs.
        \item Animals have fur.
        \item Cats have no fur.
        \item Dogs are not four-legged.
    \end{enumerate} \\ \midrule
    
    birds and fish are animals. animals have four legs. animals are normally omnivores. birds don't have four legs. fish is not an omnivore. & Does this imply that fish have four legs and birds are omnivores? & Yes   & No \newline Logical Reasoning Steps:
    \begin{enumerate}
        \item The context states that animals have four legs.
        \item Birds are animals, but they don't have four legs.
        \item Therefore, it can be concluded that not all animals have four legs.
        \item The context also states that animals are normally omnivores.
        \item Fish is an animal, but it is not an omnivore.
        \item Therefore, it can be concluded that not all animals are omnivores.
        \item Based on the reasoning steps, it cannot be implied that fish have four legs and birds are omnivores.
    \end{enumerate} \\ \midrule
    
    Blocks A and B are heavy. Heavy blocks are normally located on the table. Heavy blocks are normally red. A is not on the table. B is not red. & Does the context imply that B is on the table and A is red in color? & Yes   & No, the context does not imply that B is on the table and A is red in color.\newline{}\newline{}Logical reasoning steps:
    \begin{enumerate}
        \item The context states that heavy blocks are normally located on the table.
        \item It also states that A is not on the table.
        \item Therefore, we can conclude that A is not located on the table.
        \item The context also states that heavy blocks are normally red.
        \item It further states that B is not red.
        \item Therefore, we can conclude that B is not a heavy block.
        \item Since B is not a heavy block, it does not necessarily need to be located on the table.
        \item Additionally, the context does not provide any information about the color of A.
        \item Therefore, we cannot conclude that A is red in color.
        \item In conclusion, the context does not imply that B is on the table and A is red in color.
    \end{enumerate} \\ \bottomrule
    \end{tabular}%
    }
        \vspace{0.2cm}
    \caption{Case study on generating a logical explanation for \textit{Default Reasoning with Several Default} of \textit{Non-monotonic logic} having the worst performance by \textit{ChatGPT} in this category}
  \label{tab:appendix_explain_NM}%
\end{table*}%


==> tables/logical_PL.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \resizebox{0.85\linewidth}{!}{
    % \begin{tabular}{m{4.5cm}|m{3cm}|c|m{15.5cm}} \toprule
    \begin{tabular}{m{5cm}|m{4cm}|c|m{10cm}} \toprule
    
    Context & Question & Answer & Logical Steps \\ \midrule
    We know that atleast one of the following is true (1) she is not making a cake for the party and (2) he is writing a report for his boss. Note that we do not know which ones of (1) and (2) are true. It might be the case that only (1) is true, or only (2) is true or both are true. & If she is making a cake for the party, does this mean that he is writing a report for his boss? & Yes   & No. \newline Logical reasoning steps:     \begin{enumerate}
        \item We know that at least one of the following is true: (1) she is not making a cake for the party and (2) he is writing a report for his boss.
        \item The question asks if she is making a cake for the party, does this mean that he is writing a report for his boss?
        \item Since we do not know which one of the statements (1) and (2) is true, we cannot determine if she making a cake for the party means that he is writing a report for his boss.
        \item Therefore, the answer is No.
    \end{enumerate} \\ \midrule 
    
    We know that atleast one of the following is true (1) John is not at school and (2) Mary is taking a break from her job. Note that we do not know which ones of (1) and (2) are true. It might be the case that only (1) is true, or only (2) is true or both are true. & If John is at school, does this entail that Mary is taking a break from her job? & Yes   & No  \newline Logical Reasoning Steps:
    \begin{enumerate}
        \item We know that at least one of the following is true: (1) John is not at school and (2) Mary is taking a break from her job.
        \item If John is at school, it means that (1) is not true.
        \item Since (1) is not true, it means that Mary is not necessarily taking a break from her job.
        \item Therefore, if John is at school, it does not entail that Mary is taking a break from her job.
    \end{enumerate} \\ \midrule

    We know that atleast one of the following is true (1) Scarlett is not attending tshe lecture and (2) dani is studying for her upcoming exam. Note that we do not know which ones of (1) and (2) are true. It might be the case that only (1) is true, or only (2) is true or both are true. & If Scarlett is attending the lecture, does this mean that dani is studying for her upcoming exam?  & Yes  & No \newline Logical reasoning steps: \newline
    \begin{itemize}
        \item We know that at least one of the following is true: (1) Scarlett is not attending the lecture and (2) Dani is studying for her upcoming exam.
        \item We do not know which one of (1) and (2) is true, or if both are true.
        \item If Scarlett is attending the lecture, it means that (1) is not true.
        \item Since we do not know if (2) is true or not, we cannot conclude that Dani is studying for her upcoming exam.
        \item Therefore, we cannot say for certain if Dani is studying for her upcoming exam if Scarlett is attending the lecture.
    \end{itemize}
    \\ \midrule
    
    % We know that atleast one of the following is true (1) Levi is not studying for his exams and (2) Maya is writing a book. Note that we do not know which ones of (1) and (2) are true. It might be the case that only (1) is true, or only (2) is true or both are true. & If Levi is studying for his exams, does this mean that Maya is writing a book? & Yes  & No, if Levi is studying for his exams, it does not necessarily mean that Maya is writing a book.\newline \newline Logical Reasoning Steps:  
    % \begin{enumerate}
    %     \item Given the context, we know that at least one of the following statements is true: a) Levi is not studying for his exams. b) Maya is writing a book.
    %     \item The question asks whether if Levi is studying for his exams, it implies that Maya is writing a book.
    %     \item Since we don't have any information about the relationship between Levi studying for his exams and Maya writing a book, we cannot make a definitive conclusion.
    %     \item It is possible that Levi is studying for his exams while Maya is not writing a book. In this case, the statement "Levi is studying for his exams" does not imply that Maya is writing a book.
    %     \item It is also possible that both statements (1) and (2) are true, meaning Levi is not studying for his exams and Maya is writing a book. In this case, the statement "Levi is studying for his exams" would be false, but it still wouldn't imply that Maya is writing a book.
    %     \item Therefore, without additional information, we cannot determine a direct logical implication between Levi studying for his exams and Maya writing a book. 
    % \end{enumerate} \\ \midrule
    
    We know that atleast one of the following is true (1) Chloe is studying for her exams and (2) mila is going on vacation. Note that we do not know which ones of (1) and (2) are true. It might be the case that only (1) is true, or only (2) is true or both are true. & If Chloe isn't studying for her exams, does this entail that mila is going on vacation? & Yes   & No \newline Logical reasoning steps: 
    \begin{enumerate}
        \item We know that at least one of the following is true: (1) Chloe is studying for her exams and (2) Mila is going on vacation.
        \item If Chloe isn't studying for her exams, it means that (1) is not true.
        \item However, we don't have enough information to determine whether (2) is true or not.
        \item Therefore, we cannot conclude that Mila is going on vacation just because Chloe isn't studying for her exams.
    \end{enumerate} \\ \midrule
    
    We know that atleast one of the following is true (1) Ava is not attending the music festival and (2) she is studying for her exams. Note that we do not know which ones of (1) and (2) are true. It might be the case that only (1) is true, or only (2) is true or both are true. & If Ava is attending the music festival, does this mean that she is studying for her exams? & Yes   & No. \newline Logical reasoning steps:
    \begin{enumerate}
       \item We know that at least one of the following is true: (1) Ava is not attending the music festival and (2) she is studying for her exams.
       \item The question asks if Ava is attending the music festival, does this mean that she is studying for her exams?
        \item Since we do not know which one of the statements (1) and (2) is true, we cannot conclude that if Ava is attending the music festival, she is studying for her exams.
        \item Therefore, the answer is No.
    \end{enumerate} \\ \bottomrule
    \end{tabular}%
    }
    \vspace{0.2cm}
    \caption{Case study on generating a logical explanation for \textit{Disjunctive Syllogism} of \textit{propositional logic} having the worst performance by \textit{ChatGPT} in this category}
  \label{tab:appendix_explain_PL}%
\end{table*}%


==> tables/propositional_results.tex <==
\begin{table*}[]
\centering
\begin{tabular}{|c|cc|cc|cc|cc|}
\hline
\multirow{2}{*}{Logic Axiom}                                     & \multicolumn{2}{c|}{GPT-3}              & \multicolumn{2}{c|}{LAMA}               & \multicolumn{2}{c|}{tk-instruct}        & \multicolumn{2}{c|}{FLAN-T5}            \\ \cline{2-9} 
                                                                 & \multicolumn{1}{c|}{Accuracy} & F-score & \multicolumn{1}{c|}{Accuracy} & F-score & \multicolumn{1}{c|}{Accuracy} & F-score & \multicolumn{1}{c|}{Accuracy} & F-score \\ \hline
\begin{tabular}[c]{@{}c@{}}Modus\\ Tollens\end{tabular}          & \multicolumn{1}{c|}{94.33\%}  & 94.33\% & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       \\ \hline
\begin{tabular}[c]{@{}c@{}}Hypothetical\\ Syllogism\end{tabular} & \multicolumn{1}{c|}{97\%}     & 97\%    & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       \\ \hline
\begin{tabular}[c]{@{}c@{}}Disjunctive\\ Syllogism\end{tabular}  & \multicolumn{1}{c|}{35.55\%}  & 33.15\% & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       \\ \hline
\begin{tabular}[c]{@{}c@{}}Distructive\\ Dillema\end{tabular}    & \multicolumn{1}{c|}{90.66\%}  & 90.67\% & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       \\ \hline
\begin{tabular}[c]{@{}c@{}}Constructive\\ Dillema\end{tabular}   & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       \\ \hline
\begin{tabular}[c]{@{}c@{}}Bidirectional\\ Dillema\end{tabular}  & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       \\ \hline
\begin{tabular}[c]{@{}c@{}}Material\\ Implication\end{tabular}   & \multicolumn{1}{c|}{27.13\%}  & 25.84\% & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       \\ \hline
Commutation                                                      & \multicolumn{1}{c|}{93.66\%}  & 93.64\% & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       & \multicolumn{1}{c|}{-}        & -       \\ \hline
\end{tabular}
\caption{Evaluating LLMs on Propositional Logic.}
\end{table*}

==> tables/story_example.tex <==
\begin{table*}
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{c|m{7cm}|m{7cm}}
\toprule
Inference rules & Contxet & Story  \\ \midrule
HS & If Jerry goes for jogging, then he will work up a sweat.  If he will work up a sweat, then he will drink lots of water. & Jerry was determined to stay healthy and fit so he made sure to go for jogging every day. Sure enough, after his jogs he would work up a sweat and, in order to stay hydrated, would drink lots of water. \\ \midrule

DS  & We know that atleast one of the following is true (1) Ava is not attending the music festival and (2) she is studying for her exams. Note that we do not know which ones of (1) and (2) are true. It might be the case that only (1) is true, or only (2) is true or both are true. & Ava had an important decision to make - attend the music festival or study for her exams. She couldn't do both, so she had to choose. In the end, she decided that either she would attend the music festival or she would study for her exams - or both, but only one at a time. She wasn't sure which one she wanted to do, but she was determined to do one of them. \\ \midrule

CD   & If Lisa eats breakfast in the morning, then she will have energy to start my day. If she sleeps in late, then she will feel groggy in the morning. We know that atleast one of the following is true (1) Lisa eats breakfast in the morning and (2) she sleeps in late. Note that we do not know which ones of (1) and (2) are true. It might be the case that only (1) is true, or only (2) is true or both are true. & Lisa always faces a tough challenge every morning: eat breakfast or sleep in late. On one hand, if she eats breakfast in the morning, she will have enough energy to get her day started. On the other hand, if she sleeps in late, she will feel groggy in the morning. Despite Lisa's dilemma, one thing is for certain - either she eats breakfast or she sleeps in late.\\ \bottomrule
\end{tabular}
}
\caption{Examples of stories generated from original context for three distinct propositional rules. HS: Hypothetical Syllogism, DS: Disjunctive Syllogism, CD: Constructive Dilemma}
\label{tab:story_examples}
\end{table*}

==> tables/story_performance.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
\centering
\resizebox{0.85\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c}
    \toprule
    \multirow{2}[0]{*}{Inference Rules}  & \multicolumn{2}{c|}{Original} & \multicolumn{2}{c}{Story-like} \\ \cmidrule{2-5}
          & $A(Yes)$ & $A(No)$ & $A(Yes)$ & $A(No)$ \\  \midrule
    HS & 52.63 & 100   & 73.91 & 94.74 \\
    DS & 50.00 & 81.25 & 16.67 & 72.58 \\
    CD & 39.58 & 96.88 & 45.16 & 87.76 \\
    DD & 33.33 & 87.50 & 24.00 & 74.55 \\
    BD & 39.58 & 96.88 & 41.03 & 90.24 \\
    MT & 45.45 & 89.36 & 0     & 61.54 \\
    MI & 25.68 & 83.33 & 34.21 & 83.33 \\
    CT & 45.45 & 100   & 46.15 & 95.12 \\\midrule
    \textbf{Average} & \textbf{41.46} & \textbf{91.90} & \textbf{35.14} & \textbf{82.48}  \\ \bottomrule
    \end{tabular}%
    }
  \caption{Performance of GPT-3 given \textit{Prompt 1}(\textsection \ref{app:three_prompts}) in terms of label-wise accuracy on PL with original and story-like context from \textit{LogicBench(Eval)}.}
  \label{tab:story_perform_results}
\end{table}%

% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[htbp]
%   \centering
%   \caption{Add caption}
%     \begin{tabular}{p{4.235em}ccrr}
%     \multirow{2}[0]{*}{Rules} & \multicolumn{2}{p{8.47em}}{Original} & \multicolumn{2}{p{8.47em}}{Story} \\
%     \multicolumn{1}{r}{} & \multicolumn{1}{p{4.235em}}{A(Yes)} & \multicolumn{1}{p{4.235em}}{A(No)} & \multicolumn{1}{p{4.235em}}{A(Yes)} & \multicolumn{1}{p{4.235em}}{A(No)} \\
%     hypothetical\_syllogism & 52.63 & 100   & 73.91 & 94.74 \\
%     disjunctive\_syllogism & 50    & 81.25 & 16.67 & 72.58 \\
%     constructive\_dillema & 39.58 & 96.88 & 45.16 & 87.76 \\
%     destructive\_dillema & 33.33 & 87.5  & 24    & 74.55 \\
%     bidirectional\_dilemma & 39.58 & 96.88 & 41.03 & 90.24 \\
%     modus\_tollens & 45.45 & 89.36 & 0     & 61.54 \\
%     material\_implication & 25.68 & 83.33 & 34.21 & 83.33 \\
%     commutation & 45.45 & 100   & 46.15 & 95.12 \\
%     \textbf{Average} & \textbf{41.46} & \textbf{91.9} & \textbf{35.14} & \textbf{82.48} \\
%     \end{tabular}%
%   \label{tab:addlabel}%
% \end{table}%


==> tables/without_CoT_result.tex <==
% Table generated by Excel2LaTeX from sheet 'FLAN-T5'
\begin{table*}[htbp]
  \centering
  \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{c|c|cc|cc|cc|cc|cc}
    \toprule
     \multirow{2}[0]{*}{Type}    &    \multirow{2}[0]{*}{Rules}        & \multicolumn{2}{c|}{FLAN-T5}   & \multicolumn{2}{c|}{Tk-instruct}  & \multicolumn{2}{c|}{GPT-3} & \multicolumn{2}{c|}{ChatGPT} & \multicolumn{2}{c}{GPT-4} \\ \cmidrule{3-12}
          
    &  & $A(No)$ & $A(Yes)$ & $A(No)$ & $A(Yes)$ & $A(No)$ & $A(Yes)$ & $A(No)$ & $A(Yes)$ & $A(No)$ & $A(Yes)$  \\ \midrule 
    
    \multirow{8}[0]{*}{PL} & HS  & $100_{0.000}$     & $48.4_{0.006}$ & $97.9_{0.001}$ & $57.9_{0.052}$ & $97.6_{0.020}$ & $78.3_{0.083}$ & $100.00_{0.000}$ &$57.17_{0.016}$ & $100.00_{0.000}$ & $91.03_{0.041}$\\
    
          & DS & $64.1_{0.127}$ & $08.3_{0.144}$ & $67.9_{0.065}$ & $10.9_{0.121}$ & $75.5_{0.012}$ & $33.3_{0.577}$ & $73.77_{0.007}$ &$5.56_{0.096}$ & $100.00_{0.000}$ & $76.41_{0.072}$\\
          
          & CD  & $50.0_{0.433}$ & $25.0_{0.000}$  & $75_{0.000}$    & $25.0_{0.000}$  & $97.7_{0.019}$ & $75.4_{0.111}$ & $99.40_{0.010}$ &$81.02_{0.053}$ & $100.00_{0.000}$ & $55.74_{0.102}$ \\
          
          & DD  & $75.0_{0.000}$ & $25.0_{0.000}$   & $75.0_{0.000}$     & $25.0_{0.000}$     & $78.0_{0.022}$ & $43.4_{0.009}$  & $100.00_{0.000}$ &$33.14_{0.029}$ & $100.00_{0.000}$ & $33.22_{0.019}$\\
        
          & BD  & $75.0_{0.000}$ & $25.0_{0.000}$   & $75.0_{0.000}$     & $25.0_{0.000}$     & $80.5_{0.043}$ & $97.0_{0.052}$  & $97.38_{0.029}$ &$58.05_{0.035}$ & $100.00_{0.000}$ & $38.31_{0.023}$\\
          
          & MT  & $92.2_{0.012}$ & $44.6_{0.013}$ & $74.5_{0.019}$ & $24.4_{0.030}$ & $72.5_{0.037}$ & $17.5_{0.093}$ & $92.30_{0.014}$ &$45.47_{0.020}$ & $100.00_{0.000}$ & $70.72_{0.038}$ \\
          
          & MI & $63.6_{0.033}$ & $23.2_{0.006}$ & $64.2_{0.022}$ & $0.0_{0.000}$  & $81.5_{0.033}$ & $33.3_{0.041}$ & $91.26_{0.069}$ &$41.32_{0.054}$ & $98.81_{0.021}$  & $37.48_{0.030}$ \\
          
          & CT & $25.0_{0.433}$ & $16.7_{0.144}$ & $78.3_{0.057}$ & $31.5_{0.112}$ & $95.8_{0.038}$ & $97.0_{0.052}$ & $100.00_{0.000}$ &$52.32_{0.034}$ & $100.00_{0.000}$ & $50.24_{0.041}$ \\
          \midrule
    & \textbf{Avg}    & \textbf{$68.1_{0.130}$} & \textbf{$27.0_{0.039}$} & \textbf{$76.0_{0.020}$} & \textbf{$25.0_{0.039}$} & \textbf{$84.9_{0.035}$} & \textbf{$59.4_{0.049}$} & \textbf{$94.27_{0.016}$} &\textbf{$46.76_{0.042}$} & \textbf{$99.85_{0.003}$} &\textbf{$56.65_{0.046}$}\\
    \midrule \midrule
    
    \multirow{9}[0]{*}{FOL} & EG & $100_{0.000}$  &  $100_{0.000}$     & $95.0_{0.004}$ & $100_{0.000}$   & $88.9_{0.096}$ & $100_{0.000}$ & $89.72_{0.048}$ &$100.00_{0.000}$ & $100.00_{0.000}$ & $100.00_{0.000}$\\
    
          & UI  & $98.1_{0.032}$ & $86.9_{0.038}$ & $89.3_{0.003}$ & $84.4_{0.022}$ & $88.2_{0.042}$ & $98.2_{0.030}$ & $85.11_{0.022}$ &$94.34_{0.002}$ & $93.80_{0.025}$ &$100.00_{0.000}$\\
          
          & MP & $99.2_{0.013}$ & $79.3_{0.003}$ & $88.6_{0.010}$ & $86.3_{0.025}$ & $81.6_{0.008}$ & $82.3_{0.057}$ & $88.48_{0.044}$ &$80.09_{0.020}$ & $80.91_{0.005}$ &$95.38_{0.045}$\\
          
          & HS & $100_{0.000}$     & $49.2_{0.007}$ & $100_{0.000}$     & $52.6_{0.013}$ & $94.9_{0.028}$ & $78.7_{0.057}$ & $95.75_{0.019}$ &$53.13_{0.027}$ & $99.40_{0.010}$ &$86.99_{0.068}$\\

          & DS & $72.1_{0.052}$ & $21.9_{0.132}$ & $71.4_{0.007}$ & $04.6_{0.039}$ & $81.8_{0.034}$ & $96.3_{0.064}$ & $88.20_{0.012}$ &$97.62_{0.041}$ & $91.86_{0.016}$ &$100.00_{0.000}$\\
          
          & CD & $75.0_{0.000}$  & $25.0_{0.000}$ & $91.7_{0.144}$ & $62.0_{0.326}$ & $93.1_{0.05}$ & $65.9_{0.102}$ & $93.69_{0.040}$ &$87.95_{0.056}$ & $100.00_{0.000}$  &$79.46_{0.078}$\\
          
          & DD & $75.0_{0.000}$  & $25.0_{0.000}$     & $87.4_{0.107}$ & $28.0_{0.025}$ & $75.4_{0.004}$ & $44.4_{0.509}$ & $83.86_{0.073}$ &$30.57_{0.049}$ & $100.00_{0.000}$  &$36.64_{0.017}$\\
          
          & BD  & $25.0_{0.433}$ & $25.0_{0.000}$   & $91.7_{0.144}$ & $47.0_{0.190}$ & $77.5_{0.019}$ & $94.4_{0.096}$ & $98.75_{0.011}$ &$67.56_{0.086}$ & $100.00_{0.000}$  &$36.04_{0.024}$\\
          
          & MT & $93.3_{0.001}$ & $48.1_{0.016}$ & $81.8_{0.045}$ & $35.9_{0.050}$ & $74.8_{0.013}$ & $25.7_{0.103}$ & $85.86_{0.086}$ &$42.31_{0.133}$ & $96.75_{0.010}$ &$62.84_{0.047}$\\
          \midrule
    & \textbf{Avg}       & \textbf{$82.0_{0.059}$} & \textbf{$51.1_{0.021}$} & \textbf{$88.5_{0.051}$} & \textbf{$55.6_{0.077}$} & \textbf{$84.0_{0.033}$} & \textbf{$76.2_{0.113}$} & \textbf{$89.94_{0.039}$} &\textbf{$72.62_{0.046}$} & \textbf{$95.86_{0.007}$} &\textbf{$77.48_{0.031}$}\\
    \midrule \midrule
    
    \multirow{8}[0]{*}{NM} & DRI  & $60.4_{0.030}$ & $59.6_{0.020}$ & $52.4_{0.084}$ & $53.8_{0.081}$ & $75.0_{0.016}$ & $100_{0.000}$ & $75.63_{0.000}$ &$89.59_{0.016}$ & $69.65_{0.038}$ & $92.02_{0.010}$ \\
    
          & DRS & $66.3_{0.006}$ & $02.9_{0.025}$ & $60.0_{0.034}$ & $03.9_{0.010}$ & $72.5_{0.012}$ & $10.1_{0.036}$ & $72.72_{0.007}$ &$0.00_{0.096}$ & $72.26_{0.025}$ &$15.72_{0.055}$\\
          
          & DRD & $95.0_{0.000}$  & $95.0_{0.000}$    & $88.8_{0.036}$ & $75.7_{0.124}$ & $84.7_{0.055}$ & $100_{0.000}$ & $82.22_{0.010}$ &$100.00_{0.053}$ & $77.16_{0.053}$ &$100.00_{0.000}$\\
          
          & DRO & $40.0_{0.061}$ & $42.6_{0.023}$ & $43.8_{0.074}$ & $45.2_{0.091}$ & $65.3_{0.033}$ & $100_{0.000}$ & $70.33_{0.000}$ &$100.00_{0.029}$ & $51.30_{0.013}$ &$66.67_{0.577}$\\
          
          & RE1 & $74.2_{0.027}$ & $24.2_{0.038}$ & $85.2_{0.046}$ & $28.0_{0.009}$ & $74.3_{0.006}$ & $0.0_{0.000}$ & $81.40_{0.029}$ &$33.58_{0.035}$ & $75.00_{0.000}$ &$0.00_{0.000}$\\
          
          & RE2 & $100_{0.000}$    & $100_{0.000}$    & $98.2_{0.030}$ & $93.8_{0.053}$ & $50.0_{0.000}$ & $0.0_{0.000}$ & $62.31_{0.014}$ &$64.73_{0.020}$ & $50.00_{0.000}$ &$0.00_{0.000}$\\

          & RE3 & $65.6_{0.042}$ & $63.0_{0.019}$ & $78.2_{0.061}$ & $57.7_{0.057}$ & $64.4_{0.010}$ & $93.6_{0.055}$ & $67.21_{0.069}$ &$82.74_{0.054}$ & $69.43_{0.045}$ &$85.56_{0.019}$\\
          
          & RAP & $70.1_{0.078}$ & $62.6_{0.030}$ & $76.9_{0.021}$ & $92.5_{0.014}$ & $56.8_{0.006}$ & $92.2_{0.072}$ & $58.35_{0.000}$ &$96.97_{0.034}$ & $60.04_{0.019}$ &$100.00_{0.000}$\\
          \midrule
     & \textbf{Avg}     & \textbf{$71.4_{0.031}$} & \textbf{$56.2_{0.019}$} & \textbf{$72.9_{0.048}$} & \textbf{$56.3_{0.055}$} & \textbf{$67.9_{0.017}$} & \textbf{$62.0_{0.020}$} & \textbf{$71.27_{0.016}$} &\textbf{$70.95_{0.042}$} & \textbf{$65.61_{0.024}$} &\textbf{$57.50_{0.083}$}\\
    \bottomrule
    \end{tabular}%
    }
    \vspace{0.2cm}
  \caption{Evaluation of LLMs in terms of label-wise accuracy on \textit{LogicBench(Eval)} without chain-of-thought prompting, where $A(Yes)$ and $A(No)$ denote the accuracy for the $Yes$ and $No$ labels, respectively.}
  \label{tab:wo_cot_results}%
\end{table*}%

